The LOFAR Two Meter Sky Survey: Deep Fields, I -- Direction-dependent calibration and imaging

The Low Frequency Array (LOFAR) is an ideal instrument to conduct deep extragalactic surveys. It has a large field of view and is sensitive to large scale and compact emission. It is, however, very challenging to synthesize thermal noise limited maps at full resolution, mainly because of the complexity of the low-frequency sky and the direction dependent effects (phased array beams and ionosphere). In this first paper of a series we present a new calibration and imaging pipeline that aims at producing high fidelity, high dynamic range images with LOFAR High Band Antenna data, while being computationally efficient and robust against the absorption of unmodeled radio emission. We apply this calibration and imaging strategy to synthesize deep images of the Bootes and LH fields at 150 MHz, totaling $\sim80$ and $\sim100$ hours of integration respectively and reaching unprecedented noise levels at these low frequencies of $\lesssim30$ and $\lesssim23$ $\mu$Jy/beam in the inner $\sim3$ deg$^2$. This approach is also being used to reduce the LoTSS-wide data for the second data release.

==> DataReduction.tex <==
\section{Data Reduction}


\subsection{Direction independent calibration}

- 

\subsection{Direction dependent calibration}



==> EKF.tex <==


\section{A complex Jones-based non-linear Kalman filter}
\label{sec:EKF}

In \citet{Tasse14a} we have presented a physics-based non-linear
Kalman filter (based on the Unscented Kalman Filter) which goal was to
directly estimate the underlaying physical state of the processes
giving rise to the observed Jones matrices. The advantage of
this method was that the size of the process was orders of magnitude
lower than in Jones-based solvers, thereby improving the system's
conditioning. However the difficulty of finding physical models for
complicated effects such as the ionospheric effects at low frequency
made it complicated to use in practice. In this section we present a
Jones-based non-linear Kalman filter that aims at estimating the Jones
matrices directly (ie the net product of the physical DDE).


\subsection{Direction dependent calibration and RIME formalism}
\label{sec:Wirtinger}

A radio interferometer measures the correlation between voltages
measured between pairs of antennas. As mentioned above a series of
effects interact on the electromagnetic wave thereby changing the
properties of its coherency matrix. This has been formalised by
\citet[][]{Hamaker96} through the Radio Interferometry Measurement
Equation (RIME), that maps the sky's structure to the measured
visibilities

\begin{alignat}{2}
\label{eq:ME}
\textbf{V}_{(pq),t\nu}=& 
%\displaystyle\sum\limits_{\vec{s}}
\int_{\vec{s}}
\left(\JonesMat_{p\vec{s}t\nu}\SkyMat\ \JonesMat^H_{q\vec{s}t\nu}\right)
k^{\vec{s}}_{(pq),t\nu} \textrm{d}\vec{s}+n_{(pq),t\nu}
\\
\label{eq:kterm}
\text{with }k^{\vec{s}}_{(pq),t\nu}=&\exp{\left(-2 i\pi \frac{\nu}{c}\left(\vec{b}_{pq,t}^T(\vec{s}-\vec{s}_0)\right)\right)}\\
\text{and }\vec{b}_{pq,t}=&
\begin{bmatrix}
\u_{pq,t} \\ 
\v_{pq,t} \\ 
\w_{pq,t} 
\end{bmatrix}=
\begin{bmatrix}
\u_{p,t} \\ 
\v_{p,t} \\ 
\w_{p,t} 
\end{bmatrix}-
\begin{bmatrix}
\u_{q,t} \\ 
\v_{q,t} \\ 
\w_{q,t} 
\end{bmatrix}\\
\text{and }
\vec{s}=&
\begin{bmatrix}
\l \\ 
\m \\ 
\n 
\end{bmatrix}
\text{ and }\vec{s}_0=
\begin{bmatrix}
0 \\ 
0 \\ 
1 
\end{bmatrix}
\end{alignat}

\noindent where $\JonesMat_{p\vec{s}t\nu}$ is the Jones matrix of
antenna $p$ in direction \vec{s}, $\SkyMat$ is the four-polarization
sky matrix, $\vec{b}_{pq,t}$ is the baseline vector between antennas
$p$ and $q$, and $\vec{s}=[\l,\m,\n=\sqrt{1-\l^2-\m^2}]^T$ is a sky
direction.

Third generation calibration in radio interferometry consists in
finding the direction-time-frequency dependent Jones matrices
$\JonesMat_{p\vec{s}t\nu}$. This is traditionally done using
non-linear optimisation methods such as
Levenberg-Marquardt\footnote{See for example Black Board Selfcal (BBS)
  that uses a Levenberg-Marquardt solver to adress the
  direction-dependent calibration problem
  (\url{http://www.lofar.org/operations/doku.php?id=public:user_software:documentation:bbs}).}
or Expectation-Maximisation \citep[][]{Kazemi11}. Since these
algorithms require a Jacobian and associated Hessians to maximize an
objective function, the RIME needs to be differentiated against the
complex gains in the direction dependent Jones matrices for each given
time-frequency data chunk. This complex problem is in general treated as
real-valued by differentiating the complex variables
against real and imaginary parts.

\subsection{Wirtinger Jacobian}
\label{sec:WirtingerJacobian}

\input{WirtingerJacobian.tex}

Contrailly to {\it pealing}-like methods \citep[][]{Weeren16}, in the
familly of algorithms generated by the Wirtinger half-Jacobian described in
\ref{sec:WirtingerJacobian}, directions have to be solved for simultaneously,
on the data vector defined over a unique time and frequency
domain. While this allows for the interation between directions to be
properly taken into account, some directions with little flux will be
poorly constrained. A minimum least squares solvers such as
Levenberg-Marquardt using the half-Wirtinger Jacobian will fit
the data as best as possible with the direction-dependent model, regardless of the data's noise
properties. The poorly constrained directions will present spuriously
variable solution. In addition, the DDE calibration problem being
non-linear and often ill-conditioned, many of the 3rd generation
calibration algorithms are known to suffer from unmodeled flux absorption.

\subsection{Extended Kalman Filter}


In this section we describe an Extended Kalman Filter (EKF) that uses
the Wirtinger half-Jacobian framework described above. Contrarilly to
non-linear least squares (NLLS) iterative solvers such as LM, Kalman
filters are recursive and Bayesian, with the covariance of the process
and data vectors being used and updated along the recurtion
(technically, they minimise the mean square error). While a NLLS
solver will create unphysical jumps in the estimated process due to
thermal noise and ill-conditioning, a Kalman filter will create smooth
solutions.

However, the Kalman filter is designed for systems where the
measurement (mapping the process to the data vector) and evolution
operators are linear. In the case of the DDE calibration problem, the
measurement operator is non linear while the evolution operator is
unknown (especially when elements such as ionospheric distortion come
into play). Similarly to NLLS solvers that use a Jacobian to linearise the
problem, non-linear Kalman filters can be formulated for mildy
non-linear systems. 



In the following, we assume an evolution operator
$\textbf{x}_{k}=\textbf{f}(\textbf{x}_{k-1})+\textbf{w}_k$ describing
the evolution of the physical quantities underlying the RIME, and a
measurements operator
$\textbf{y}_{k}=\textbf{h}(\textbf{x}_k)+\textbf{v}_k$ generating the
set of measurement for a given process vector $\textbf{x}_k$ (examples for
both $\textbf{f}$ and $\textbf{h}$ are given in Sect. \ref{sec:Simulations}). The random
variables $\textbf{v}_k $ and $\textbf{w}_k$ model the noise and are
assumed to follow normal distributions $\textbf{v}_k \sim
\mathcal{N}(0, \textbf{R}_k)$ and $\textbf{w}_k \sim\mathcal{N}(0,
\textbf{Q}_k)$, where $\textbf{R}_k$ and $\textbf{Q}_k$ are the data
and process covariance matrix respectively. In the following, we name
the {\it predicted-process} and {\it data} domains the
codomains of $\textbf{f}$ and $\textbf{h}$, respectively.

The traditional Kalman filter \citep{Kalman60} assumes (a) $\textbf{f}$ and $\textbf{h}$ to
be linear operators (written $\textbf{F}$ and $\textbf{H}$ below for
$\textbf{f}$ and $\textbf{h}$ respectively). If the process vector $\textbf{x}_{k-1}$ for the time-step $k-1$ has
$\hat{\textbf{x}}_{k-1\mid k-1}$ estimated mean and
$\textbf{P}_{k-1\mid k-1}$ estimated covariance from the data at step
$k-1$, assuming (b) Gaussian noise in the process and data domains,
$\textbf{x}_{k-1\mid k-1}$ is distributed following
$\textbf{x}_{k-1 \mid k-1}\sim\mathcal{N}(\hat{\textbf{x}}_{k-1\mid k-1},
\textbf{P}_{k-1 \mid k-1})$.

Under the conditions (a) and (b), operators $\textbf{F}$ and $\textbf{H}$ yield Gaussian distributions
in the predicted-process and data domains respectively. Given
$\hat{\textbf{x}}_{k-1\mid k-1}$ and $\textbf{P}_{k-1 \mid k-1}$ the
Kalman filter (i) predicts $\hat{\textbf{x}}_{k\mid k-1}$ and
$\textbf{P}_{k \mid k-1}$ through $\textbf{F}$, and (ii) updates those
to $\hat{\textbf{x}}_{k\mid k}$ and
$\textbf{P}_{k \mid k}$ through $\textbf{H}$ given the data
$\textbf{y}_{k}$.

It can be shown that the mean and covariance of $\textbf{x}_{k-1}$ can
be evolved through $\textbf{F}$ giving $\hat{\textbf{x}}_{k\mid k-1}$
and $\textbf{P}_{k\mid k-1}$ as follows:

%\begin{align}
%\begin{split}
\begin{alignat}{2}
\label{eq:KF_xf}
%\hat{\textbf{x}}_{k\mid k-1} &= \textbf{F}_{k}\hat{\textbf{x}}_{k-1\mid k-1} + \textbf{B}_{k} \textbf{u}_{k-1}\\
\hat{\textbf{x}}_{k\mid k-1} &= \textbf{F}_{k}\hat{\textbf{x}}_{k-1\mid k-1} \\
\label{eq:KF_Pf}
\textbf{P}_{k\mid k-1} &=  \textbf{F}_{k} \textbf{P}_{k-1\mid k-1} \textbf{F}_{k}^{\text{T}} + \textbf{Q}_{k}.
\end{alignat}
%\end{split}
%\end{align}

\noindent Taking into account the data vector $\textbf{y}_k$ at step $k$, the
updated mean and covariance $\hat{\textbf{x}}_{k\mid k}$ and
$\textbf{P}_{k|k}$ of $\textbf{x}_k$ are estimated through the
calculation of the {\it Kalman gain} $\textbf{K}_k$, and are given by


%\begin{align}
%\begin{split}
\begin{alignat}{2}
\label{eq:KF_Sk}
\textbf{S}_k &= \textbf{H}_k \textbf{P}_{k\mid k-1} \textbf{H}_k^\text{T} + \textbf{R}_k \\
\label{eq:KF_Kk}
\textbf{K}_k &= \textbf{P}_{k\mid k-1}\textbf{H}_k^\text{T}\textbf{S}_k^{-1}\\
\tilde{\textbf{y}}_k &= \textbf{y}_k - \textbf{H}_k\hat{\textbf{x}}_{k\mid k-1}\\
\hat{\textbf{x}}_{k\mid k} &= \hat{\textbf{x}}_{k\mid k-1} + \textbf{K}_k\tilde{\textbf{y}}_k\\
\textbf{P}_{k|k} &= (I - \textbf{K}_k \textbf{H}_k) \textbf{P}_{k|k-1},
\end{alignat}
%\end{split}
%\end{align}


The estimate $\hat{\textbf{x}}_{k\mid k}$ is
optimal in the sense that $\textbf{P}_{k \mid k}$ is minimized. This approach is extremely powerful for linear-systems, but the radio
interferometry measurement equation is highly non-linear (the operator
$\textbf{h}$ in Eq. \ref{eq:ME}). This makes the
traditional Kalman filters unpractical for the radio interferometry
calibration problem.



==> HalfWSolver.tex <==
\section{Half Wirtinger Solver}

\large{\textbf{[There are a lot of missing steps in the following -
      only the main steps are given. Actually, giving all the step
      would take like 5 more pages... Additionally, I've made a lot of very
      detailed tests to check that this is indeed exactly what's
      happening. In the following $\L=L^H$]. I only consider the gains
    (source of 1Jy at the phase center). But it also works with
    arbritrary skymodel.}}

\def\VDataResid{\vec{\mathrm{v}}_r}
\newcommand{\N}[1]{|#1|^2}
\newcommand{\Cell}[2]{\left[#1\right]_{#2}}
\def\Sum{\displaystyle\sum}

Let's consider a Gauss-Newton algorithm based on the Wirtinger
Jacobian. The update at step $k+1$ is written as

\def\dg{{\bm{\delta g}}}
\def\dgh{{\bm{\delta g}_h}}


\begin{alignat}{2}
%\bm{g}_{k+1}&=\bm{g}_{k}+\dg\\
\begin{bmatrix}
\bm{g}\\ 
\conj{\bm{g}}
\end{bmatrix}_{k+1}&=
\begin{bmatrix}
\bm{g}\\ 
\conj{\bm{g}}
\end{bmatrix}_{k}
+
\begin{bmatrix}
\dg\\ 
\conj{\dg}
\end{bmatrix}
\\
\label{eq:BlockGN}
\nonumber\mathrm{with\ }\delta\bm{g}&=\left(\Jacob^H\Jacob+\sigma \Unity\right)^{-1}_{LL}\Lb\VDataResid\\
&+\left(\Jacob^H\Jacob+\sigma \Unity\right)^{-1}_{LR}\Rb\VDataResid
\end{alignat}

\noindent and the half Jacobian update step is written as

\begin{alignat}{2}
\dgh&=\left(\Lb\L\right)^{-1}\Lb\VDataResid
\end{alignat}

In this section we will show that under a few reasonable assumptions
we have

\begin{alignat}{2}
\label{eq:gamma}
\dg&=\frac{1}{2}\dgh
\end{alignat}

Since the Hessian can be written as 

\begin{alignat}{2}
\label{eq:facet}
\Jacob^H\Jacob=&
\begin{bmatrix}
\Lb\L+\sigma\Unity&\Lb\R\\ 
\Rb\L&\Rb\R+\sigma\Unity\\ 
\end{bmatrix}
\end{alignat}

\noindent the blocks $LL$ and $RL$ of the inverse of the Hessian can be written as

\def\A{{\Lb\L}}
\def\Ai{\left(\A\right)^{-1}}
\def\Aireg{\left(\A+\sigma \Unity\right)^{-1}}
\def\B{{\Lb\R}}
\def\Bh{{\Rb\L}}
\def\Teq{\Lb\L-\Rb\L\Aireg\Lb\R+\sigma\Unity}
\def\C{\Aireg\B\bm{\mathrm{T_1}}^{-1}}
\def\T1{{\bm{\mathrm{T}}_{\sigma}}}
\def\Tz{{\bm{\mathrm{T}}_{0}}}


\begin{alignat}{2}
\label{eq:facet}
\left(\Jacob^H\Jacob\right)^{-1}_{LL}=&\Aireg+\bm{\mathrm{C}}\Bh\Aireg\\
\left(\Jacob^H\Jacob\right)^{-1}_{LR}=&-\bm{\mathrm{C}}\\
\mathrm{with\ }\mathrm{\bm{C}}=&\C\\
\label{eq:DefT1}
\mathrm{and\ }\T1=&\Teq
\end{alignat}

%% \noindent giving

%% \def\T{\bm{\mathrm{T}}}

%% \begin{alignat}{2}
%% \gamma=&1+\left(\dgh^H\dgh\right)^{-1}\dg^H\T\dgh\\
%% \mathrm{with\ }\T=&\Lb\T_0\R\T^{-1}_1\Rb\L\Ai\\
%% \T_0=&\L\Aireg\Lb-\Unity\\
%% \end{alignat}

If $\sigma$ is small we have

\begin{alignat}{2}
\Aireg&\sim\Ai\left(\Unity-\sigma \Ai\right)
\end{alignat}

\noindent and expending Eq. \ref{eq:BlockGN} we get

\begin{alignat}{2}
%\dg=&\left(\Unity+\sigma\Ai\right)\dgh\\
%&-\sigma\Ai\left(\Unity+\sigma\Ai\right)\Lb\R\T1^{-1}\Rb\L\Ai\dgh\\
\label{eq:dg}
\dg\sim&\dgh-\sigma\Ai\Lb\R\T1^{-1}\Rb\L\Ai\dgh\\
\nonumber
\mathrm{with\ }{\T1}=&\Lb\L-\Rb\L\Ai\Lb\R\\
\label{eq:Tsigma}&+\sigma\left(\Rb\L\left(\A\right)^{-2}\Lb\R+\Unity\right)
\end{alignat}

\noindent In the direction independent and unpolarised case, if $P=\Sum_i\N{g_i}$ and
$\Diracb{i}{j}=1-\Dirac{i}{j}$, a cell $\{ij\}$ of $\T1$ can be written as

\begin{alignat}{2}
\label{eq:DefT}
\nonumber
\T1|_{ij}=&\delta_{ij}h_i
-g_j \conj{g_i} \Sum_{p}\N{g_p}h_p^{-1}\Diracb{i}{p}\ \Diracb{j}{p}\\
&+\sigma
\left(
\delta_{ij}+g_j\conj{g_i}\Sum_{p}\N{g_p}h_p^{-2}\Diracb{i}{p}\ \Diracb{j}{p}
\right)
\end{alignat}

where  $P=\Sum_{i}\N{g_i}$ if the total power received by the antennas and $h_p=P-\N{g_p}$.

In order to find in which regime Eq. \ref{eq:gamma} is true, we
will show the following



\begin{enumerate}[(i)]
\item $\T1$ is singular if $\sigma=0$ and specifically
  $\dim{\ker{\T1}}=1$. The consequence is that the Gauss-Newton
  algorithm has to be regularised (using a non-zero $\sigma$).
\item If $\sigma\ll 1$ and $\sigma\neq 0$, $\T1^{-1}\sim\left(2\sigma\sqrt{\vec{g}^H\vec{g}}\right)^{-1}\vec{\conj{g}}\vec{g}^T$
\end{enumerate}

\subsubsection{If $\sigma=0$ then $\dim{\ker{\T1}}=1$}

In this sections we show that (i) $\Tz$ is singular and that (ii) its
null-space is 1-dimentional. In order to show (i), and instead of
expliciting the eigenvector and eigenvalues of $\Tz$ (which would be
rather tedious), we can prove that $\conj{\vec{g}}$ is an eigenvector
in the null space $\Tz\conj{\vec{g}}=\vec{0}$. Specifically, if
$f_p=\N{g_p}h_p^{-1}$ we have

\begin{alignat}{2}
-\frac{\Cell{\Tz\conj{\vec{g}}}{i}}{\conj{g_i}}=&
\N{g_i}-P + \Sum_{jp}\N{g_j}f_p\Diracb{i}{p}\ \Diracb{j}{p}\\
\nonumber
=&\N{g_i}-P \\
\nonumber
&+ \Sum_{jp}\N{g_j}f_p-\Sum_{j}\N{g_j}f_j\\
&-f_i\Sum_{j}\N{g_j}+f_i\N{g_i}\\
=&\Sum_{jp}\left(\N{g_j}f_p-\N{g_j}f_p\Dirac{j}{p}\right)-P\\
=&\Sum_{p}\left(f_p\Sum_{j}\N{g_j}\Dirac{j}{p}\right)-P\\
=&0
\end{alignat}


Therefore
$\vec{u}_0=\conj{\vec{g}}/\sqrt{P}$ is an eigenvector of $\Tz$ and has a
corresponding null eigenvalue.

In the following, we show that the null space of $\Tz$ is 1-dimentional. Since $\Tz$ is hermitian, we can prove that if
there is an eigenvector $\vec{u}_1$ such that $\vec{u}_1^H\Tz\vec{u}_1=0$
and $\vec{u}_0^H\vec{u}_1=0$ then $\vec{u}_1=\vec{0}$ (eigenvectors of Hermitian matrices are orthogonal), thereby showing
that $\dim{\ker{\Tz}}=1$.

Specifically, if $\vec{u}$ is the given eigen vector in the null space we have

\begin{alignat}{2}
\Cell{\Tz \vec{u}}{i}=&
-\left(P-\N{g_i}\right)u_i + \conj{g_i}\Sum_{jp}g_ju_jf_p\Diracb{i}{p}\ \Diracb{j}{p}\\
\nonumber
=&-\left(P-\N{g_i}\right)u_i + \conj{g_i}\Sum_{jp}g_ju_jf_p \\
&- \conj{g_i}\Sum_{j}g_ju_jf_j - \conj{g_i}f_i\Sum_{j}g_ju_j + \N{g_i}f_iu_i
\end{alignat}

\noindent and 

\begin{alignat}{2}
\nonumber
\vec{u}^H\Tz \vec{u}=&
\Sum_{i}-\left(P-\N{g_i}\right)\N{u_i} + \sum_{i}\conj{u_i}\conj{g_i}\Sum_{jp}g_ju_jf_p\\
&+\N{g_i}\N{u_i}f_i\\
\label{eq:Positivity}
=&\Sum_{i}\N{u_i}\left(P-\N{g_i}\right)P\left(P-2\N{g_i}\right)
\end{alignat}

\noindent Since $P-\N{g_i}>0$, $P>0$ and if $P-2\N{g_i}>0$ if the
interferometer has more than two antennas, then in order to fullfil
\ref{eq:Positivity} we must have $\vec{u}=\vec{0}$.


%Since finding closed form for the eigen vectors and eigen values of
%$\T1$ is difficult, we first show that  In a first step we will show that $\T$ is non-singular only if
%$\sigma\neq 0$


\subsubsection{Estimating $\T1^{-1}$}

Now computing the eigenvalues and eigenvectors for non-zero $\sigma$,
and since $\sigma\ll 1$, writting $f'_p=\N{g_p}h^{-2}_p$, the perturbed lowest eigen value can be written as

\begin{alignat}{2}
\lambda/\sigma=&\vec{g}^T\Rb\L\left(\A\right)^{-2}\Lb\R\conj{\vec{g}}+1\\
=&
1+\Sum_{jp}\N{g_j}f'_p\Diracb{i}{p}\ \Diracb{j}{p}
\\
=&1+\Sum_{jp}\N{g_j}f'_p-\Sum_{j}\N{g_j}f'_j\nonumber \\
&-f'_i\Sum_{j}\N{g_j}+\N{g_i}f'_i
\end{alignat}


Expliciting Eq. \ref{eq:Tsigma} and assuming the power received by each antenna is similar
$\alpha\sim\N{g_i},\ \forall i$ we get


\begin{alignat}{2}
\lambda=2\sigma
\end{alignat}

Since $\sigma$ is arbritrarilly small and $\dim{\ker{\Tz}}=1$ we have 

\begin{alignat}{2}
\T1^{-1}\sim\left(2\sigma\right)^{-1}\vec{u}_0\vec{u}_0^H
\end{alignat}

\noindent and since $\VDataResid=\L\vec{g}=\R\vec{\conj{g}}$,
refactoring Eq. \ref{eq:dg} we get 

\begin{alignat}{2}
\dg=\frac{1}{2}\dgh
\end{alignat}

\large{\textbf{So.... In that case of a 1Jy source at the phase
    center, direction independent, if all antennas receiving the same
    power, the half jacobian LM with lambda=1 does the same as a full
    Jacobian Gauss Newton!!!}}



==> Implementation.tex <==
\section{Implementation and simulation}

\subsection{Adaptative step}

\subsection{Update P}

\subsection{Iterative EKF}



==> Introduction.keep.tex <==
\section{Introduction}

The new generation of radio interferometers aim at producing
sensitive, high resolution, and high dynamic range images over large
fields of view. However the combination of these specifications
require to calibrate and compensate for the many antenna, time,
frequency and direction-dependent Jones matrices that disturb the
sources' electo-magnetic coherency. These effects include (i) the
ionosphere frequency dependent phase shifts and (ii) Faraday rotation,
(iii) the station beam, or the pointing errors. Calibration consists
in estimating the Jones matrices inverting a large system of
measurement equations, that model the mappings between the sky's
struture and the visibility measurements (ie the correllation of
woltages between pairs of antennas). The radio interferometry
measurement equation (RIME) has been discussed in much detail in
\citet[][and references therein]{Hamaker96,Oleg11}. While estimating
the direction-independent Jones matrices is well understood for
decades, the calibration of direction-dependent effects (DDE
calibration or third generation calibration) is difficult in terms of
(i) algorithmic complexity and (ii) stability since the DD-RIME system
is often ill conditioned.

Various approaches have been proposed in the last decade to adress DDE
calibration. One can classify calibration algorithms into two
famillies. The first aims at estimating the physical parameters
underlaying the Jones matrices (the {\it physics-based} solvers), for
example the values of a the clock shift or an electron density in the
ionosphere \citep[see][for a review of DI and DD
  solvers]{Tasse14a}. The strength of these approaches is that the
number of parameters to be estimated is much less thereby improving
conditioning and algorithmic cost. However, the instrumental effects
in the RIME have to be physically modeled to very high accuracy -
which can be extremely difficult in some cases (ionospheric
scintillation, antenna coupling, etc). The second familly of
algorithms ({\it Jones-based}) aim at estimating the effective Jones
matrices \citep[see][and references
  therein]{Yatawatta08,Noordam10,Smirnov15}. Contrarilly to the
physics-based, the Jones-based solvers do not need accurate modeling,
but dependending on the number of free parameters can suffer from
ill-conditioning issues. In the most extreme cases, thermal noise can
be fitted, leading to fake high dynamic range, or unmodeled
astrophysical flux absorption.

In this paper we aim at adressing the issues of conditioning in the
framework of DD Jones-based calibration. Specifically, we follow on
\citet{Tasse14b} and \citet{Smirnov15} that have proposed a
computationally effiscient Jones-based solver which structure is based
on recent results in the field of complex optimisation (based on the
so-called Wirtinger derivates). In addition we have shown in \citet{Smirnov15}
that the algorithm presented by \citet{Salvini14} was a a special case
of a Wirtinger solver with a single direction. 



==> MODS.tex <==
\subsubsection{Multi-Object Dynamic Spectro-Polarimetry}
\label{sec:MODS}

%\COMMENT{Tim}{Is this section moving to another paper? If not then we should stick an example spectrum in this paper}

In this section we describe a new technique that we use to extract
dynamic spectra from the interferometric data. It is indeed
scientifically interesting to study flux density variation in 
time-frequency space. While extragalactic
sources are not expected to vary significantly within a typical 8
hours \LoTSS/ scan, Galactic objects such as pulsars, stars or
exoplanets can show quickly varying flux density. The inverse \RIME/
tells us that each synthesised beam (in the dirty
or residual image) can be seen as the weighted sum of all visibilities.
In order to image all pixels for all times and frequencies, in the case of \LoTSS/ we would have to estimate 
$n_\nu\times n_t \times n_{pix}^2$ pixels (with
$(n_\nu,n_t,n_{pix})=(480,3600,2.10^4)$), making this operation
prohibitive.

Instead, we propose to select $n^{sel}_{pix}=10^{2-3}$ directions of
interest in any given \LoTSS/ field and image $n_\nu\times n_t \times n^{sel}_{pix}$ pixels. This
technique resembles Multi-Object Spectroscopy, widely used in the
optical and near infrared energy domains, where a limited number of fibers are put in the
focal plane of telescopes to aquire spectra. Applied to radio
interferometry, we can extend the technique to dynamic
spectro-polarimetry (estimating the IQUV Stokes parameters for all
available times and frequencies).

One of the difficulties of image synthesis with interferometric data as
compared to optical telescopes is the sparse coverage of the
uv-domain. This implies that images as built by Fourier-transforming
the visibilities in the uv-domain need to be deconvolved in
order to interpret flux densities. The \PSF/ is indeed non-zero even
far from its origin, and sources cross contaminate each other. The
situation is even worse when synthesising images over narrow
time-frequency domains where the uv-coverage is poor. Basically a pixel
mapped in a given direction in the time-frequency space would
have the contribution of all time-frequency sidelobes of all sources
in the field leaking onto it.

\def\BL{{(pq),t\nu}}
\def\BLpq{{\vec{b}^{t\nu}_{pq}}}
\def\BL{{\vec{b}}}
\def\Vres{{\bm \delta}^{\textbf{v}^{c}}_\BL}

To tackle this issue, in Multi-Object Dynamic Spectro-polarimetry
(MODS) we make the reasonalble assumption that most of the
time-frequency varying sources are compact (the peak flux in the
residual image is then interpretable as a physical integrated flux density), and we work on the residual visibilities on a baseline $\BL$

\begin{alignat}{2}
\label{eq:ResVis}
\Vres =&\textbf{v}^{c}_\BL-
\int_{\vec{s}}
\widehat{\MuellerMat^{\vec{s}}_{\bl}}
\MuellerMatBeam^{\vec{s}}_{\bl}\textbf{x}_{\vec{s}\nu}
k^{\vec{s}}_{\bl} \textrm{d}\vec{s}
\end{alignat}

\noindent where 
$\widehat{\textbf{x}_{\vec{s}\nu}}$ and
$\widehat{\MuellerMat^{\vec{s}}_{\bl}}$ are the sky model and Mueller
matrices as estimated by Alg. \ref{alg:DR2}. The polarimetric dynamic spectrum
$\textbf{x}_{\vec{s},t\nu}$ in a given direction $\vec{s}$ is then
built as

\def\Dxtnu{{\bm \delta}^{\textbf{x}}_{\vec{s},t\nu}}

\begin{alignat}{2}
\label{eq:DynSpec}
%\left<\widehat{\textbf{x}_{\vec{s},t\nu}}\right>=&
\widehat{\textbf{x}_{\vec{s},t\nu}}=&\widehat{\textbf{x}_{\vec{s},\nu}}+{\bm \delta}^{\textbf{x}}_{\vec{s},t\nu}\\
\text{with } \Dxtnu=&
\displaystyle\sum\limits_{(pq)} \widehat{\MuellerMatBeam_\BLpq}^{-1} \widehat{\MuellerMat_\BLpq}^{-1} {\bm \delta}^{\textbf{v}^{c}}_\BLpq
\conj{k^{\vec{s}}_\BLpq}
\end{alignat}

\noindent where the term $\Dxtnu$ is an IQUV-pixel for a given
direction $\vec{s}$, time $t$ and frequency $\nu$. It is the phased sum of all
visibilities corrected in that direction.

%% This step is labeled as Step
%% 3.6 in 

%% \COMMENT{Martin}{Not finished? Or just need to add a reference?}




==> ModelingDDE.tex <==
\section{Improving calibration robustness}



- Measurement equation

- effect of sky incompleteness

\subsection{Amplitude fitting}

\subsection{Phase fitting}

\subsection{Holes}


==> Observations.tex <==

\input{Tables/TabObs.tex}


==> SourceCounts.tex <==
\section{Source counts}

\subsection{Systematics}


==> Symbols.tex <==
\newcommand{\MyWidthH}{.8\columnwidth}

\begin{table}[t]\footnotesize
  \caption{\label{tab:symbols} Overview of the mathematical notation used throughout this paper}
\begin{tabular}{l@{~~}p{\MyWidthH}}
\midrule%\\%\hline\\
$\JonesMat^{\vec{s}}_{pt\nu}$\dotfill&  Direction dependent $2\times2$ complex Jones matrix. It varies over direction $\vec{s}$, antenna $p$, time $t$, and frequency $\nu$.\\
$\JonesMatDI_{pt\nu}$\dotfill& Direction independent Jones matrix\\
$\MuellerMat^{\vec{s}}_{\vec{b}t\nu}$\dotfill&  Direction dependent Mueller matrix\\
$\MuellerMatDI$\dotfill&  Direction independent Mueller matrix\\
$\OpIm$\dotfill& The imaging function abstracting the call to our direction dependent imager \DDFacet/. It maps a set of visibility $\mathbf{v}$ and Jones matrices estimates $\widehat{\JonesMat}$ to a wide band sky model $\widehat{\vec{x}_\nu}$ \\
$\OpCal$\dotfill& The calibration function that abstracts the call to the direction dependent calibration algorithm implemented in \kMS/. It maps the set of visibilities $\textbf{v}$, the estimates beam $\JonesMatBeam_{\Omega_n}$, the skymodel $\widehat{\SkyXnu}$ to the estimated set of Jones matrices $\widehat{\JonesMat}$. The Jones matrices are estimated over piecewise the constant domains $\Delta t$, $\Delta \nu$ and $\Omega_n$ being the time, frequency and direction axes respectively.\\
$\OpNorm$\dotfill& The function that normalises the Jones matrices (only used in \PipeVI/).\\
$\OpFit$\dotfill& The function that fits the Jones matrices' phase and amplitudes (only used in \PipeVII/ and discussed in detail in Sec. \ref{sec:regularisation}).\\
$\OpBoot$\dotfill& The function that bootstraps the flux scale.\\
$\OpClust$\dotfill& The function that spatially tesselates the domains for the piecewise constant Jones matrices estimates. It maps the sky model to a set $\Omega$ of $(\l,\m)$ directions.\\
$\varphi$\dotfill& The function that sets the amplitude of a scalar
Jones matrix to unity. It is used for phase-only calibration. \\
\bottomrule
\end{tabular}
\end{table}



